Waves in ice

Ocean surface waves can propagate long distances through regions containing floating ice covers. The impacts ocean waves have on the ice covers are of interest in the climate change era, as the polar regions experience pressure from rising temperatures. This chapter provides a review of observations and theoretical models for ocean wave propagation through the marginal ice zone, landfast ice and ice shelves. It traces the historical evolution of the field, from seminal work in the 1970s-80s up to recent research advances. Key research questions are identified for each of the three ice covers, and commonalities between them are highlighted. The chapter concludes with perspectives and outlooks on the field of waves in ice, in the context of the dramatic changes currently occurring to the world's sea ice and ice shelves.

==> boxes-luke.tex <==
%% BOXES

\usepackage{tcolorbox}% http://ctan.org/pkg/tcolorbox
\definecolor{mycolor}{rgb}{0.122, 0.435, 0.698}% Rule colour
\makeatletter
\newcommand{\tbox}[5]{
\setbox0=\hbox{#1}%
\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
\begin{tcolorbox}[colback=#3,colframe=#4,
      boxrule=#5,arc=4pt,
      left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt,
      width=#2]   %\@tempdima]
    #1
\end{tcolorbox}}
\makeatother

\NewDocumentCommand\mybox{om}{%
\IfNoValueTF{#1}{
\tbox{#2}{\textwidth}{white}{mycolor}{2pt}
}{
\tbox{#2}{#1}{white}{mycolor}{2pt}
}}

%\NewDocumentCommand\mytitlebox{om}{%
%\IfNoValueTF{#1}{
%\tbox{#2}{\textwidth}{gray!30}{mycolor}{0pt}
%}{
%\tbox{#2}{#1}{gray!30}{mycolor}{0pt}
%}}
%
%\NewDocumentCommand\myparbox{om}{%
%\IfNoValueTF{#1}{
%\tbox{#2}{\textwidth}{blue!10}{white}{0pt}
%}{
%\tbox{#2}{#1}{blue!10!white!90}{white}{0pt}
%}}
